Computational Security Analysis of the UMTS and LTE Authentication and Key Agreement Protocols

We present a computational security analysis of the Authentication and Key Agreement (AKA) protocols for both Long-Term Evolution (LTE) and Universal Mobile Telecommunications System (UMTS). This work constitutes the first security analysis of LTE AKA to date and the first computationally sound analysis of UMTS AKA. Our work is the first formal analysis to consider messages that are sent in the core network, where we take into account details of the carrying protocol (i.e., MAP or Diameter) and of the mechanism for secure transport (i.e., MAPsec/TCAPsec or IPsec ESP). Moreover, we report on a deficiency in the protocol specifications of UMTS AKA and LTE AKA and the specifications of the core network security (called network domain security), which may enable efficient attacks. The vulnerability allows an inside attacker not only to impersonate an honest protocol participant during a run of the protocol but also to subsequently use wireless services on his behalf. UMTS AKA run over MAP with MAPsec seems vulnerable in the most straight-forward application of the attack. On the other hand, our analysis shows that UMTS and LTE AKA over Diameter/IPsec and UMTS AKA over MAP/TCAPsec (with sufficiently long session identifiers) computationally satisfy intended authentication properties as well as some key secrecy properties, assuming that the used primitives meet standard cryptographic assumptions.

==> conclusion.tex <==
We present the first computational security analysis of the Authentication and Key Agreement  of UMTS and LTE, where we consider entity authentication and key secrecy properties while taking into account the carrying protocols within the core network.
The analysis uncovers a flaw in the specifications of UMTS and LTE AKA  and the network domain security with rather serious consequences. An outside attacker can defeat entity authentication of the user equipments to the serving networks. And an inside attacker can authenticate as another honest subscriber to a serving network and use the wireless services on his behalf. 
Previous published analyses of UMTS AKA were working in a purely symbolic model and did not catch the attacks because they generally made too strong assumptions on the connection between serving network and home network. 
%The attacks are not prevented by anything stated in the specifications.

%The attacks are possible because the specification are not sufficiently precise with respect to 
%A critical weakness of the specifications of the security architectures for UMTS/ LTE AKA  \cite{ts33.102,ts33.401} (and GSM SIA \cite{ts42.009,ts43.020}) is that they do not explicitly detail which security requirements are necessary for the channels between serving networks and home networks. In particular, detailing or requiring a way to bind an authentication data request to the correct user equipment, which must be protected, is missing in the specifications of UMTS/LTE AKA. 
%Instead, the specifications refer to the specifications \cite{ts33.210,ts33.310,ts33.200}, where, for the case of SS7-based connections or IP-based inter-domain connections, it is not ensured  whether security goals defined there are the right ones for UMTS/LTE AKA (note session IDs are not mentioned at all). 
The attacks can be prevented if the carrying protocols use unique integrity-protected session identifiers in the communication between serving and home network. In practice, UMTS AKA is vulnerable if it is run over MAP and MAPsec, as the session identifiers are not integrity-protected, while UMTS and LTE AKA run over the Diameter protocol and IPsec are secure. 
We use the tool CryptoVerif to verify entity authentication properties and key secrecy properties with respect to the computational model for the UMTS and LTE AKA protocols when unique session IDs and authenticated encryption in the core network are used.  
%Our analysis shows that for IP-based connections, IPsec in combination with the usage of different ports for different session does protect the protocol against our attacks, but this is on a level of detail not covered by the specifications. And for SS7-based connections, MAPsec in combination with unique invoke IDs for each authentication data request also protects our attacks; but this too is on a level of detail not covered by the specifications. 
%Furthermore, in the case of IP-based intra-domain connections, the specifications leave the security assumptions entirely unspecified and up to each operator to choose.  %At the same time the exchange between serving network and home is presented in \cite{ts33.102,ts33.401} in a way that implicitly assumes  perfect security of the communication channel. 
%

We question whether it is prudent practice to make the security  of the UMTS/LTE AKA protocol  (or, in fact, any other cryptographic protocol) %implicitly 
reliant on the carrying protocols and their protection without considering the security of the combined protocol. %stating it explicitly. %; these details are unusually low level for a protocol description.  %correct IPsec EPS protocol deployment as a necessary requirement for the security. 
Instead we believe that it would be much more desirable to directly consider the combination of AKA with carrying protocol and its protection.  The UMTS/LTE AKA protocols should ideally be strengthened by making the binding of $H$'s authentication data response for an intended $U$ explicit in the AKA specifications  %We are working on a design for this.  % and we think that is a dubious security practice to rely on IPsec without even stating what functionalities IPsec should offer, as has been done in this case of AKA. 
%Notice also that, for intra-domain connections, operators may implement their proprietary solutions instead of using IPsec or MAPsec. Therefore, correcting the UMTS/ LTE AKA protocol directly (\eg \ by including the IMSI in the authentication data response) will also better assist operators  who wish to employ secure proprietary solutions for intra-domain connections. 
%
%Moreover, our analysis shows that the gap in the specification can be exploited even by an outside attacker. 
%An inside attacker may successfully impersonate an honest user $U$ while $U$ is not present at the same time. 
%However, we have not yet experimented with implementations of this attack. 
%
%The UMTS/LTE AKA (and GSM SIA) protocol specifications can be corrected by properly binding the authentication data response to the user equipment in the corresponding request 
and by {explicitly} requiring that authenticated encryption is used to protect the connection between serving and home network. 
Moreover, the specifications \cite{ts33.102} and \cite{ts33.401} of UMTS/LTE AKA need to be revised so that  the desired security properties on all connections are explicitly stated. This is also important for intra-domain connections, where operators are free to implement proprietary solutions and may currently  miss to implement or sufficiently protect  mechnisms for the serving network to correctly match the authentication data responses, even if their implementation is guided by the specifications of the security architecture \cite{ts33.102,ts33.401}.
%We suggest corrections to the protocols and w

 %(unless it is \emph{a priori} prevented  through missing entity authentication or through the use of the exchanged keys during the protocol execution) are satisfied. 
%Our proofs are to a large extend not fully automatic.
%
%Item for inclusion: 
%The LTE authentication protocol is relying on the underlying IPsec for security. 
%The AKA protocol should be secure in itself.  Also something to do with minimality of solutions.
%
%Besides properly binding the responses of the home network to the requests or users, it also seems inevitable that the specifications \cite{ts33.102} and \cite{ts33.401} of UMTS/LTE AKA (and \cite{ts42.009,ts43.020} of GSM SIA) need to be revised so that  the security assumptions on all connections are explicitly stated.  %For UMTS/LTE AKA the proper binding of the authentication data requests has to be established. 
%This is also important for intra-domain connections, where operators are free to implement proprietary solutions and may currently  miss to implement or sufficiently protect  instruments for the serving network to correctly match the authentication data responses, even if their implementation is guided by the specifications of the security architecture \cite{ts33.102,ts33.401}. 
%
%We are currently extending our CryptoVerif analysis to the corrected GSM SIA protocol.

We are interested in further exploring %, ideally in cooperation with 3GPP and mobile network operators, 
to what extend real-world systems are vulnerable to our attack, which, \eg, also depends on how widely MAPsec or TCAPsec with short transaction identifiers are deployed in practice.  We would also like to expand  our analysis to scenarios of the protocol execution that are not covered in the present work, \eg\ the scenarios that are related to the use of TMSIs, and include the usage of the sequence number in order to verify stronger authentication properties than entity authentication. Moreover, it would be interesting to verify under which conditions the specified MILENAGE algorithms and the key derivation algorithm satisfy the computational assumptions made in this work.
%Moreover, it would be interesting to obtain  not only asymptotic security guarantees but also exact security guarantees with respect to the (fixed) key lengths used in the specifications of UMTS and LTE AKA. CryptoVerif already gives exact security bounds with respect to security parameters, so a promising strategy for us seems to be to take CryptoVerif transformations and exact success probabilities for the last games and extend these to the full security proofs.

%\jkt{improve design of UMTS and LTE AKA}

\subsubsection{Acknowledgements} We thank Valtteri Niemi and Steve Babbage for helpful discussions on the feasibility of the session-mixup attack. And we thank Bruno Blanchet for helping to automate the proofs for entity authentication of the user to the serving network. 


==> intro.tex <==
%\subsection{Motivation}

%It is exciting times in mobile networks.  
These are exciting times in the development of mobile networks.
The GSM %Global System for Mobile communication (GSM) 
and UMTS mobile networks are a worldwide success with now about 6 billion %users 
supscriptions \cite{userconnections2011},
and still growing. The pace of innovation in mobile terminal hardware and software is amazing, where touch screen and online packet switched internet access have become a consumer standard.  New mobile systems are rolled out, which include the 3GPP recent developments named 'Long Term Evolution' (LTE) and 'System Architecture Evolution'  (SAE).  The new system is called 'Evolved Packet System (EPS), emphasizing the all-IP packet switching design throughout the system unto the user's mobile terminal.  Although EPS is the proper technical term for this new 3GPP mobile system generation of SAE/LTE, we will keep with the most well-known name LTE. %Our analysis includes the existing UMTS because the security architecture and protocols of LTE are based on and compatible with the UMTS security architecture.  
% Should we mention something on LTE Advanced here?
%
There is a multitude of security issues in such large networked systems.  Here we will focus on the mobile terminal access security 
by means of an authentication and key agreement protocol (AKA) that is structured very similar in UMTS and LTE.  
%
%We have managed to introduce many acronyms already in this paper.  The specifications of 3GPP is brimful with abbreviations and acronyms.  Possibly this is for good reasons, but nevertheless, the unlike naming of  similar elements and functionality of the architecture in GSM, UMTS, and LTE makes it hard to read, and becomes a source of potential confusion, though their abstracted functionalities are much the same. (For instance, the core packet switching element of GSM is SGSN, whereas that of UMTS is MSC, and that of LTE is MME. ) We will try to keep the use of these acronyms to a minimum.
%
% \jkt{Shall we note that we will call the EPS AKA simply \emph{LTE AKA}, that's perhaps less confusing and we can always talk about UMTS \& LTE AKA}
The technical problem we are addressing is to find out whether the UMTS AKA and LTE AKA are secure with respect to the \emph{Computational Model}, \ie \ the security model that is used in \emph{Modern Cryptography} \cite{GoMi_82,GoMi_84}. %, and  we do this by deploying CryptoVerif. 
This work constitutes the first computational analysis of both UMTS AKA and LTE AKA. While there exist formal analyses of UMTS AKA in the \emph{Symbolic Model} of security (also called the \emph{Dolev-Yao} model and inspired by \cite{DolevYao83}), it is in fact the first security analysis of LTE AKA to date. 
%This work provides the first security proofs of the UMTS and LTE AKA protocols that are sound with respect to the computational model. %In doing so  this work provides the first computationally sound proofs for both UMTS AKA and LTE AKA. 
While there exist already formal security proofs for UMTS AKA in the symbolic model, this work provides the first security proofs for LTE AKA to date. 
Although the design of LTE AKA is based on UMTS AKA, its security can a priori not be deduced from the security properties of UMTS AKA as, for instance, the LTE AKA protocol has been designed to offer stronger authentication guarantees.
Furthermore, our proofs are the first that cover the AKA\footnote{We sometimes write only \emph{AKA} when we talk about both UMTS AKA and LTE AKA } messages sent within the core networks, where we take into account security details of the protocols over which the UMTS and LTE AKA protocol messages are transported. Namely, our proofs examine security properties of the UMTS and LTE AKA protocol for the scenario with the strongest protection described in the UMTS and LTE specifications: within the core network, the AKA messages are carried over the Mobile Application Part (MAP) protocol~\cite{ts29.002} or the Diameter protocol~\cite{ts29.272,rfc3588} and are additionally protected via MAPsec~\cite{ts33.200} or TCAPsec~\cite{ts33.204} (which is the descendant of MAPsec) or IPsec ESP~\cite{ts33.210}.
%
%as described in the UMTS and LTE specifications, within the core network, the AKA messages are carried over the Mobile Application Part (MAP) protocol~\cite{ts29.002} or the Diameter protocol~\cite{ts29.272,rfc3588} and are additionally protected via TCAPsec~\cite{ts33.204} (which is the descendant of MAPsec~\cite{ts33.200}) or IPsec ESP~\cite{ts33.210}. 
We note that there are scenarios where the 3GPP specifications~\cite{ts33.210,ts33.200,ts33.204} allow network operators to use their proprietary solutions for protecting core network messages or where the AKA protocols can be executed without any confidentiality protection. 
Proprietary solutions can generally not be verified unless explicit details are given\footnote{We do not have any knowledge about proprietary solutions (and their specifics) for protecting core network AKA messages that deviate from the strongest protection described in the specifications. (and considered in this work)}. % the network users  can only hope that they are secure\
And in the case that no confidentiality protection is used in the core network, the exchanged session keys are exposed and can be eavesdropped, and so there are no meaningful security properties to prove.



%\begin{comment}
Designing security protocols has proven to be a very error-prone task. There exist many examples of security protocols that were believed to be secure, usually with respect to the symbolic or the computational model of security, 
but that were later shown to be flawed (often in its logical structure) \cite{Lowe1995,Meadows1999IKE,Mitchell1998,CervesatoICarspa}. Especially ensuring the security of a protocol under concurrent executions of multiple protocol sessions (\emph{runs}) is a challenging task in analyzing security protocols by hand. Therefore, considerable effort has been directed towards the development of tools that can analyze security protocols in an automatic fashion. 
There are already several tools that are able to analyze security protocols with respect to the symbolic model. %(also called \emph{Dolev-Yao} model). 
In particular secrecy and authentication properties, even of complex protocols, can be shown with a high degree of automation. But also other properties, \eg \ privacy and verifiability properties of electronic voting protocols, can be handled by such symbolic provers \cite{scytherthesis,cav05avispa,isabelle,BlanchetCSFW01,Meadows96b}. 
While attacks found against protocols within the symbolic model, where cryptographic primitives are perfectly secure, immediately translate to attacks in the computational model, it is not clear what the successful verification of a protocol in the symbolic model signifies when the security of the protocol is considered in the more fine-grained computational model where an adversary may attack a protocol via the used primitives. %Consequently, security proofs in the computational model are preferable over those in the symbolic model.
In order to take advantage of the existing effective tools that work in the symbolic model but, at the same time, obtain the stronger security guarantees of the computational model, a line of research focuses on so-called \emph{Computationally Sound} frameworks, \eg \ \cite{BaPW4_03,Canetti06,DattaCSFW06,CKW-jar2010,ComonHagiyaKawamotoSakurada12ispec}. %In such frameworks, proofs are conducted in the symbolic model, but the results are sounds with respect to the computational model given that the used cryptographic primitives are sufficiently strong (\eg \ public-key encryption usually has to be IND-CCA secure). 
However, currently such frameworks lack the tool support yet which would allow proofs without a lot of user interaction. In recent years, an alternative direction has been taken by building tools that prove the security of protocols or cryptographic primitives directly in the computational model \cite{BlanchetTDSC07,Barthe:2011:CRYPTO}. One such solution, CryptoVerif, has previously been applied to obtain mechanized security proofs in the computational model of complex real-world protocols such as Kerberos  \cite{BlanchetJST08} or TLS \cite{Bhargavan:2008}.
%\end{comment}

We also conduct our analysis of UMTS AKA and LTE AKA with CryptoVerif. 
Our results are twofold: On the one hand, we discover a previously undetected vulnerability in the specifications of  both UMTS AKA and LTE AKA  and the specifications of the core network security~\cite{ts33.210,ts33.200,ts33.204}.  Due to  an identity misbinding of the authentication vectors an attacker can execute a parallel session attack.\footnote{We note that the attack is also relevant for the cases where the protocol messages of the GSM Subscriber Identity Authentication \cite{ts43.020,ts42.009} are meant to be protected within the  core network (cf. Appendix~\ref{app:gsmsia}).}
%Strictly speaking, GSM SIA also suffers from essentially the same vulnerability, although this case is more ambiguous than UMTS or LTE as we explain below. 
%This paper focuses mainly on UMTS and LTE and deals with GSM  rather on the side. We also do not perform a CryptoVerif analysis of GSM SIA.
The vulnerability found could be exploited by both outside and inside attackers in order to break authentication of a user to a serving network. Furthermore, inside attackers may impersonate an honest user and use wireless services on his behalf without the user being present on the network at that time. %The attack may have gone undetected as teh
We reported the vulnerability to the 3GPP in Spring 2012 and have since been waiting for any reply. 
In practice, UMTS AKA over MAP/MAPsec is flawed as the session identifiers (called \emph{TCAP transaction identifier}) are not protected. And the attack may also be effective against both UMTS AKA and LTE AKA over intra-domain, depending on the proprietary security solutions in place. %Furthermore, UMTS AKA over MAP/TCAPsec may be vulnerable if the session identifier are not sufficiently long.
%We have not tested current implementations for susceptibility to these attacks (cf. Section \ref{subsec:connassump}).  
%We propose a simple correction to  UMTS/LTE AKA and use CryptoVerif to proof correspondence properties (implying entity authentication) and also some secrecy properties for the session key (where possible). 

On the other hand, our analysis shows that UMTS and LTE AKA run over Diameter/IPsec EPS  and UMTS over MAP/TCAPsec are computationally secure: 
%Using this tool we discover a previously undetected vulnerability in the specifications of  both UMTS AKA and LTE AKA. %which is due to  an identity misbinding of the authentication vectors. 
%We note that the specifications of the GSM SIA protocol \cite{ts43.020,ts42.009} suffer, strictly speaking, from the same vulnerability (cf. Section~\ref{sec:gsmSia}).
%Strictly speaking, GSM SIA also suffers from essentially the same vulnerability, although this case is more ambiguous than UMTS or LTE as we explain below. 
%This paper focuses mainly on UMTS and LTE and deals with GSM  rather on the side. We also do not perform a CryptoVerif analysis of GSM SIA.
%The vulnerability can be exploited by both outside and inside attackers in order to break authentication of a user to a serving network. Furthermore, inside attackers may impersonate an honest user and use wireless services on his behalf without the user being present on the network at that time. %The attack may have gone undetected as teh
%We reported the vulnerability to the 3GPP where the issue is currently under investigation. We have not tested current implementations for susceptibility to these attacks (cf. Section \ref{subsec:connassump}).  
Under standard assumptions on the cryptographic primitives, \eg,  including IND-CPA secure symmetric encryption and WUF-CMA secure integrity protection, and under the additional assumption that the session identifier used in the carrying protocols (MAP or Diameter) are unique with overwhelming probability, we %propose a simple correction to  UMTS/LTE AKA and 
use CryptoVerif to prove intended authentication properties %(via correspondence assertions) 
and secrecy properties for the session keys that are exchanged with the AKAs. 
%We note that if the session identifier are not unique then an implementation of AKA may be vulnerable to a recently discovered parallel session attack~\cite{TsayMjol_LTEattack2012} (see next section and Section~\ref{sec:attack}).


\subsubsection{Related Work}
%Astonishingly, no security analysis in any form has been published on the LTE AKA to date, while rather few analyses have been published on the UMTS AKA. 

%There are two analysis works contained in the 3GPP technical report TR33.902 (2001)~\cite{3GformalAna}.  Annex A documents a formal analysis of the 3G authentication protocol using TLA (Temporal Logic of Actions) as a specification language.  The focus of the analysis is on what happens in case of failure of synchronicity of the sequence number SQN between the user terminal and the home network.  The assumption is that the mobile station works correctly, but the authentication vectors sent from the home network might get lost somehow.  No cryptographic property in the standard sense is modeled.
Annex B of the 3GPP technical report TR33.902 (2001)~\cite{3GformalAna} documents a formal analysis of the UMTS AKA protocol using %an AUTLOG specification (
a BAN logic variant, \ie, a symbolic and not computational analysis.  The analysis %finds everything in order 
verifies authentication and secrecy properties under the assumption that the home network acts as a trusted third party. 
The flaw that we present here is not detected in \cite{3GformalAna} because strong assumptions (called \emph{ prerequisites on SN's side}) are used which already eliminate the weakness in the protocol and the network domain security.
%\jkt{The BAN logic analysis of AKA, which actually disregards the authentication data request, uses strong prerequisites on SN's side, section 3.1.1, which already bind H's response to U. Therefore they don't find our attack }  
%For instance, the user has to trust that fresh random numbers and keys are generated by the home network. 
%This analysis is purely symbolic, whereas our analysis reported here is based on computational models of the cryptographic primitives. 

The GSM  Subscriber Identity Authentication protocol does not provide for the authentication of the access network, which obviously creates a problem with detecting false base stations. The interoperability of the GSM and UMTS systems perpetuates this attack possibility, reported in~\cite{Meyer:2004:MAU:1023646.1023662}.  Our analysis is not directed to the problems of interoperability between LTE/UMTS/GSM.

\cite{TangNW11} formally analyze the security UMTS and GSM roaming protocols using the tool ProVerif~\cite{BlanchetCSFW01} with respect to the symbolic security model. Again, they use strong assumptions on the core network communication between serving networks and home networks (namely, they use private channels), which cause them to overlook the vulnerability we discover.

A redirection attack on the UMTS AKA is reported in~\cite{ZhangFang05}, which  exploits the observation that the user is not able to authenticate the identity of the \emph{serving} network because this is not included in the authentication vector provided by the home network.  The new LTE AKA specification that we analyze is designed to fix this weakness and implicitly authenticate the serving network to the user.

A recent paper focuses on the unlinkability and anonymity properties of the protocol~\cite{Ryan2011}.  They also use the ProVerif tool for a symbolic analysis, and the paper describes an attack that enables the adversary to distinguish a known user from any other.  This is done by replaying captured messages from the known user and use the different error messages that are returned. The analysis models the UMTS AKA as a simplified two-party protocol between a user and the core network. However, by reducing UMTS AKA to a two-party protocol, the weakness uncovered in the present work is stamped out. % which uses a three-party model and, therefore, stays closer to the protocol specifications.

Our work is also relevant for RFC 4187 \cite{rfceapaka} that specifies an \emph{Extensible Authentication Protocol Method for 3rd Generation Authentication and Key Agreement (EAP-AKA)} based on UMTS AKA, which is compatible with \cite{rfceap}. In particular, close attention needs to be paid in case the communication between EAP authenticator and authentication server should be secured. We note that the  authors of \cite{rfceapaka} explicitly state that the IETF has not validated the security claims.

\subsubsection{Structure of this work}
In Section~\ref{sec:prot}, we will give an overview of the Mobile Network architecture and give a description of %GSM SIA, 
the UMTS AKA and LTE AKA protocols. In Section~\ref{sec:attack}, we describe the vulnerability we found on both 
%GSM SIA, as well as 
on the specifications of UMTS and LTE AKA and its consequences. %, where we describe the relevance of the vulnerability for GSM SIA in Section~\ref{sec:gsmSia}. \ 
In Section~\ref{sec:ana}, we present our computational security proofs of UMTS and LTE AKA using the tool CryptoVerif. Finally, we conclude with Section~\ref{sec:conc}.


==> macros-cv.tex <==
\newcommand{\ab}{\allowbreak}

%Syntax of games

\newcommand{\parpop}{\mid}
\newcommand{\alet}[2]{{#1} := {#2};}
\newcommand{\repl}[2]{{}!^{{#1}\leq{#2}}}
\newcommand{\cinput}[2]{#1(#2)}
\newcommand{\coutput}[2]{\overline{#1}\langle #2 \rangle}
\newcommand{\cin}[1]{\cinput{c}{#1}}
\newcommand{\cout}[1]{\coutput{c}{#1}}
\newcommand{\fun}[3]{({#1}) \rightarrow_{#2} {#3}}

\newcommand{\kw}[1]{\mathsf{#1}}
\newcommand{\kwf}[1]{\mathrm{#1}}
\newcommand{\vn}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\rn}[1]{\textbf{#1}}


\newcommand{\IF}{\kw{if}}
\newcommand{\THEN}{\kw{then}}
\newcommand{\ELSE}{\kw{else}}
\newcommand{\FIND}{\kw{find}}
\newcommand{\SUCHTHAT}{\kw{suchthat}}
\newcommand{\NEW}{\kw{new}}
\newcommand{\NEWCHANNEL}{\kw{newChannel}}
\newcommand{\LET}{\kw{let}}
\newcommand{\IN}{\kw{in}}
\newcommand{\EVENT}{\kw{event}}
\newcommand{\IEVENT}{\kw{inj\text{-}event}}
\newcommand{\assign}[2]{\LET\ #1 = #2\ \IN\ }
\newcommand{\bassign}[2]{\LET\ #1 = #2}
\newcommand{\Res}[2]{\NEW \ {#1}:{#2}}
\newcommand{\Reschan}[1]{\NEWCHANNEL\ {#1}}
\newcommand{\baguard}[1]{\IF\ {#1}\ \THEN\ }
\newcommand{\bguard}[3]{\baguard{#1}{#2}\ \ELSE\ {#3}}
\newcommand{\kevent}[1]{\EVENT\ {#1}}
\newcommand{\kfun}{\kw{fun}}
\newcommand{\bafind}[3]{\FIND \ {#1}\ \SUCHTHAT \ \kw{defined}({#2})\fand {#3}\ \THEN\ }
\newcommand{\orfind}[3]{\oplus\ {#1}\ \SUCHTHAT \ \kw{defined}({#2})\fand {#3}\ \THEN\ }
\newcommand{\bfind}[5]{\bafind{#1}{#2}{#3}{#4}\ \ELSE\ {#5}}
\newcommand{\cfind}[7]{\FIND \ (\mathop{\textstyle\bigoplus}\nolimits_{#1}^{#2} {#3}\ \SUCHTHAT \ \kw{defined}({#4})\fand {#5}\ \THEN\ {#6})\ \ELSE\ {#7}}
\newcommand{\cdfind}[7]{\FIND \ (\mathop\bigoplus\nolimits_{#1}^{#2} {#3}\ \SUCHTHAT \ {#4}\fand {#5}\ \THEN\ {#6})\ \ELSE\ {#7}}
\newcommand{\defined}{\kw{defined}}
\newcommand{\bitstringset}{\mathit{Bitstring}}
\newcommand{\bitstring}{\mathit{bitstring}}
\newcommand{\blocksize}{\mathit{blocksize}}
\newcommand{\sblocksize}{\mathit{sblocksize}}
\newcommand{\bitstringbot}{\mathit{bitstring}_{\bot}}
\newcommand{\injbot}{\kwf{i}_{\bot}}
\newcommand{\maxmac}{\mathit{maxmac}}
\newcommand{\macs}{\mathit{macs}}
\newcommand{\maxenc}{\mathit{maxenc}}
\newcommand{\seed}{\mathit{seed}}
\newcommand{\mkeyseed}{\mathit{mkeyseed}}
\newcommand{\mkey}{\mathit{mkey}}
\newcommand{\keyseed}{\mathit{keyseed}}
\newcommand{\key}{\mathit{key}}
\newcommand{\nonce}{\mathit{nonce}}
\newcommand{\prpckeyseed}{\mathit{prpckeyseed}}
\newcommand{\prpckey}{\mathit{prpckey}}
\newcommand{\prpckuh}{\mathit{prpckuh}}
\newcommand{\prfkeyseed}{\mathit{prfkeyseed}}

\newcommand{\constone}{\mathit{const}_{1}}
\newcommand{\consttwo}{\mathit{const}_{2}}
\newcommand{\constthree}{\mathit{const}_{3}}
\newcommand{\constfour}{\mathit{const}_{4}}


\newcommand{\vKhost}{\mathit{Khost}}
\newcommand{\vKkey}{\mathit{Kkey}}
\newcommand{\vKmkey}{\mathit{Kmkey}}
\newcommand{\vLhost}{\mathit{Lhost}}
\newcommand{\vLkey}{\mathit{Lkey}}
\newcommand{\vLmkey}{\mathit{Lmkey}}

\newcommand{\prpkuh}{\mathit{prpKuh}}
\newcommand{\prfkuh}{\mathit{prfKuh}}
\newcommand{\prfkey}{\mathit{prfkey}}

\newcommand{\rksh}{\mathit{rKsh}}
\newcommand{\ksh}{\mathit{Ksh}}
\newcommand{\mksh}{\mathit{mKsh}}


\newcommand{\bool}{\mathit{bool}}
\newcommand{\true}{\kwf{true}}
\newcommand{\false}{\kwf{false}}

\newcommand{\Adv}{{\cal A}}

\newcommand{\secp}{\eta} % security parameter
\newcommand{\obssecp}{\rightsquigarrow_{\secp}}

\newcommand{\fand}{\wedge}
\newcommand{\for}{\vee}
\newcommand{\fnot}{\neg}

\newcommand{\prpcblocksize}{\mathit{prpcblocksize}}


% Function symbols for Kerberos


\newcommand{\fmac}{\mathrm{mac}}
\newcommand{\fcheckmac}{\mathrm{checkmac}}
\newcommand{\fmkgen}{\mathrm{mkgen}}

\newcommand{\fprpckgen}{\mathrm{prpckgen}}
\newcommand{\fprpcenc}{\mathrm{prpcenc}}

\newcommand{\fprfkgen}{\mathrm{prfkgen}}



\newcommand{\fprf}{\mathrm{prf}}

\newcommand{\fenc}{\mathrm{enc}}
\newcommand{\fdec}{\mathrm{dec}}
\newcommand{\finjbot}{\mathrm{injbot}}
\newcommand{\fkgen}{\mathrm{kgen}}


\newcommand{\fpkgen}{\mathrm{pkgen}}
\newcommand{\fskgen}{\mathrm{skgen}}
\newcommand{\fpenc}{\mathrm{penc}}
\newcommand{\fpdec}{\mathrm{pdec}}

\newcommand{\fspkgen}{\mathrm{spkgen}}
\newcommand{\fsskgen}{\mathrm{sskgen}}
\newcommand{\fsign}{\mathrm{sign}}
\newcommand{\fcheck}{\mathrm{check}}

\newcommand{\fkeyderiv}{\mathrm{keyderivation}}


\newcommand{\fconcatone}{\mathrm{concat}_{1}}
\newcommand{\fconcattwo}{\mathrm{concat}_{2}}
\newcommand{\fconcatthree}{\mathrm{concat}_{3}}
\newcommand{\fconcatfour}{\mathrm{concat}_{4}}
\newcommand{\fconcatfive}{\mathrm{concat}_{5}}
\newcommand{\fconcatsix}{\mathrm{concat}_{6}}
\newcommand{\fconcatseven}{\mathrm{concat}_{7}}
\newcommand{\fconcateight}{\mathrm{concat}_{8}}
\newcommand{\fconcatnine}{\mathrm{concat}_{9}}











% --------------------------------------------------------------------- %
% Typesetting definitions:              Sample output:                  %
%                                                                       %
% \begin{defn}                                                          %
% \categ{M,N}{terms}\\          M, N ::=        terms           %
% \entry{x}{variable}\\                   x               variable      %
% \entry{M\ N}{application}\\             M N             application   %
% \entry{\lambda x.\ M}{abstraction}      \x.M            abstraction   %
% \end{defn}                                                            %
%                                                                       %
% This is a tabbing environment; the last entry should have no \\.      %
% --------------------------------------------------------------------- %

\newenvironment{defn}{\begin{tabbing}
  \hspace{1.5em} \= \hspace{.36\linewidth - 1.5em} \= \hspace{1.5em} \= \kill
%  \hbra\\[-.8ex]
  }{
%\\[-.8ex]\hket
  \end{tabbing}}
\newenvironment{shortdefn}{\begin{tabbing}
  \hspace{1.5em} \= \hspace{.30\linewidth - 1.5em} \= \hspace{1.5em} \= \kill
%  \hbra\\[-.8ex]
  }{
%\\[-.8ex]\hket
  \end{tabbing}}
\newcommand{\entry}[2]{\>$#1$\>\>#2}
\newcommand{\clause}[2]{$#1$\>\>#2}
\newcommand{\categ}[2]{\clause{#1::=}{#2}}
\newcommand{\subclause}[1]{\>\>\>#1}



\newcommand{\ev}{E}
\newcommand{\evseq}{{\cal E}}
\newcommand{\adeftest}[1]{\baguard{\defined ({#1})}}
\newcommand{\venv}{\rho}
\newcommand{\ltr}[1]{\mathrel{\xrightarrow{#1}}}
\newcommand{\evalterm}{\Downarrow}
\newcommand{\red}[2]{\ltr{#1}_{#2}}
\newcommand{\redq}{\rightsquigarrow}
\newcommand{\redsecp}[2]{\ltr{#1}_{\secp,#2}}
\newcommand{\initconfig}{\mathrm{initConfig}}
\newcommand{\config}{\mathbb{C}}
\newcommand{\fc}{\mathrm{fc}}
\newcommand{\kvar}{\mathrm{var}}
\newcommand{\fevent}[1]{\EVENT(#1)}
\newcommand{\fievent}[1]{\IEVENT(#1)}
\newcommand{\step}{\tau}


==> umtsMacros.tex <==


